PARAM-1 BharatGen 2.9B Model

Large Language Models (LLMs) have emerged as powerful general-purpose reasoning systems, yet their development remains dominated by English-centric data, architectures, and optimization paradigms. This exclusionary design results in structural under-representation of linguistically diverse regions such as India, where over 20 official languages and 100+ dialects coexist alongside phenomena like code-switching and diglossia. We introduce PARAM-1, a 2.9B parameter decoder-only, text-only language model trained from scratch with an explicit architectural and linguistic focus on Indian diversity. PARAM-1 is trained on a bilingual dataset consisting of only Hindi and English, constructed with a strong focus on fact-rich, high-quality content. It is guided by three core principles: equitable representation of Indic languages through a 25% corpus allocation; tokenization fairness via a SentencePiece tokenizer adapted to Indian morphological structures; and culturally aligned evaluation benchmarks across IndicQA, code-mixed reasoning, and socio-linguistic robustness tasks. By embedding diversity at the pretraining level-rather than deferring it to post-hoc alignment-PARAM-1 offers a design-first blueprint for equitable foundation modeling. Our results demonstrate that it serves as both a competent general-purpose model and a robust baseline for India-centric applications.

==> large_tables/table_routing_examples.tex <==
\begin{table*}[t]
    \centering
    %\small
    \scalebox{0.8}{
    % \begin{tabular}{lll}
    \begin{tabular}{ll}
    \toprule
    Task & Question and generation \\   
    \midrule
    GSM8K & \makecell[l]{Q: \underline{\color{blue}{Jan}\color{magenta}{et}\color{blue}{’}}\color{orange}{s} \color{black}{}\underline{\color{magenta}{ducks lay}} \color{orange}{1}\color{black}{}\underline{\color{magenta}{6 eggs} \color{blue}{per} \color{magenta}{day}}\color{cyan}{.} \color{black}{}\underline{\color{blue}{She e}}\color{orange}{ats} \color{black}{}\underline{\color{magenta}{three for breakfast}} \color{cyan}{every} \color{black}{}\underline{\color{magenta}{morning}} \color{cyan}{and} \color{black}{}\underline{\color{magenta}{bakes muff}}\color{orange}{ins} \color{black}{}\underline{\color{blue}{for}}\\ \color{black}{}\underline{\color{blue}{her} \color{magenta}{friends} \color{blue}{every} \color{magenta}{day}} \color{cyan}{with} \color{black}{}\underline{\color{magenta}{four.} \color{blue}{She s}\color{magenta}{ells the remainder} \color{blue}{at} \color{magenta}{the farmers' market}} \color{cyan}{daily for} \color{black}{}\underline{\color{magenta}{\$}}\color{orange}{2} \color{black}{}\underline{\color{magenta}{per fresh}}\\ \color{black}{}\underline{\color{magenta}{du}}\color{orange}{ck} \color{black}{}\underline{\color{magenta}{egg}}\color{red}{.} \color{black}{}\underline{\color{cyan}{How}} \color{orange}{much} \color{black}{}\underline{\color{magenta}{in dollars} \color{blue}{does she} \color{teal}{make} \color{blue}{every}} \color{orange}{day} \color{black}{}\underline{\color{blue}{at the} \color{magenta}{far}}\color{orange}{mers' market}\color{cyan}{?}\\  
    A: \underline{\color{blue}{Jan}}\color{orange}{et}\color{black}{}\underline{\color{magenta}{’}}\color{orange}{s} \color{black}{}\underline{\color{magenta}{du}}\color{orange}{cks} \color{black}{}\underline{\color{magenta}{lay}} \color{orange}{16 eggs} \color{red}{per} \color{orange}{day}. \color{black}{}\underline{\color{blue}{She e}}\color{orange}{ats} \color{black}{}\underline{\color{magenta}{three}} \color{red}{for} \color{orange}{breakfast} \color{red}{every} \color{orange}{morning}\color{cyan}{.} \color{black}{}\underline{\color{blue}{So she has}} \color{orange}{1}\color{black}{}\underline{\color{magenta}{6} \color{teal}{-}} \color{orange}{3} \color{black}{}\underline{\color{magenta}{=}}\\ \color{orange}{13} \color{black}{}\underline{\color{magenta}{eggs} \color{blue}{left. She} \color{magenta}{b}}\color{orange}{akes} \color{red}{m}\color{orange}{uffins} \color{black}{}\underline{\color{blue}{for}} \color{red}{her} \color{black}{}\underline{\color{magenta}{friends}} \color{red}{every} \color{orange}{day} \color{teal}{with} \color{orange}{4}\color{black}{}\underline{\color{magenta}{.}} \color{red}{So she} \color{teal}{has} \color{orange}{13} \color{black}{}\underline{\color{teal}{-}} \color{orange}{4 = 9} \color{black}{}\underline{\color{magenta}{eggs}} \color{red}{left.} \color{black}{}\underline{\color{blue}{She}}\\ \color{black}{}\underline{\color{teal}{s}}\color{orange}{ells} \color{black}{}\underline{\color{blue}{the}} \color{orange}{remainder} \color{red}{at the} \color{black}{}\underline{\color{magenta}{far}}\color{orange}{mers'} \color{black}{}\underline{\color{teal}{market}} \color{red}{daily} \color{cyan}{for} \color{black}{}\underline{\color{teal}{\$}}\color{orange}{2 per fresh duck egg}\color{red}{.} \color{black}{}\underline{\color{blue}{So she has}} \color{orange}{9} \color{black}{}\underline{\color{teal}{*}} \color{orange}{2} \color{black}{}\underline{\color{magenta}{=}} \color{orange}{18} \color{black}{}\underline{\color{magenta}{dollars}\color{blue}{.}}\\ \color{black}{}\underline{\color{blue}{The}} \color{orange}{answer} \color{cyan}{is} \color{orange}{18.}} \\
    \hline
    Human Eval & \makecell[l]{Q: \color{red}{from typing import} \color{blue}{List}\\ \\ \color{black}{}\underline{\color{teal}{def has\_close}\color{orange}{\_}\color{teal}{elements(numbers: List[float}\color{orange}{],} \color{teal}{threshold:} \color{cyan}{float}\color{orange}{)}\color{teal}{-> bool}\color{orange}{:}}\\    
    \quad \color{black}{}\underline{\color{teal}{""" Check if in given list}} \color{blue}{of} \color{black}{}\underline{\color{teal}{numbers}}\color{blue}{,} \color{black}{}\underline{\color{teal}{are any}} \color{magenta}{two} \color{black}{}\underline{\color{teal}{numbers closer}} \color{blue}{to} \color{magenta}{each} \color{red}{other} \color{blue}{than} \\
    \quad \color{black}{}\underline{\color{teal}{given threshold.}}\\ 
    \quad \color{black}{}\underline{\color{teal}{> > > has}}\color{red}{\_close\_}\color{blue}{elements}\color{black}{}\underline{\color{teal}{([1.0}\color{orange}{,} \color{teal}{2}\color{orange}{.0, 3.0],} \color{teal}{0}\color{orange}{.}\color{teal}{5)}}\\
    \quad \underline{\color{teal}{False}}\\
    \quad \underline{\color{teal}{> > > has}\color{cyan}{\_close}}\color{red}{\_}\color{black}{}\underline{\color{cyan}{elements}\color{orange}{([}\color{teal}{1}\color{orange}{.0,} \color{teal}{2}\color{orange}{.8}\color{teal}{, 3}\color{orange}{.}\color{teal}{0}\color{orange}{,} \color{teal}{4}\color{orange}{.}\color{teal}{0,} \color{orange}{5.0}\color{teal}{,} \color{orange}{2}\color{teal}{.}\color{orange}{0}\color{teal}{],}} \color{red}{0}\color{black}{}\underline{\color{teal}{.}\color{orange}{3)}}\\
    \quad \underline{\color{orange}{True}}\\
    \quad \underline{\color{orange}{"""}}\\
    A: \underline{\color{teal}{for} \color{teal}{i} \color{teal}{in}} \color{red}{range}\color{black}{}\underline{\color{orange}{(}\color{teal}{len}\color{orange}{(}}\color{red}{numbers}\color{black}{}\underline{\color{teal}{)} \color{teal}{-} \color{orange}{1}\color{orange}{):}}\\
    \quad \underline{\color{teal}{for} \color{teal}{j} \color{orange}{in} \color{blue}{range}\color{orange}{(}\color{teal}{i} \color{teal}{+}} \color{red}{1}\color{black}{}\underline{\color{orange}{,} \color{teal}{len}\color{orange}{(}}\color{blue}{numbers}\color{black}{}\underline{\color{teal}{)):}}\\
    \quad \quad \underline{\color{teal}{if} \color{teal}{abs}\color{teal}{(}\color{teal}{numbers}\color{orange}{[}\color{orange}{i}\color{orange}{]} \color{orange}{-} \color{orange}{numbers}\color{cyan}{[j]}\color{orange}{)} \color{teal}{< threshold}\color{orange}{:}}\\
    \quad \quad \quad \underline{\color{teal}{return} \color{cyan}{True}}\\
    \underline{\color{teal}{return} \color{cyan}{False}}}\\
    \hline
    \makecell[l]{Natural\\ Questions} & \makecell[l]{Q: \underline{\color{cyan}{who} \color{blue}{got} \color{red}{the first no}}\color{magenta}{bel prize} \color{black}{}\underline{\color{blue}{in}} \color{magenta}{physics}\\ 
    A: \underline{\color{red}{Max}} \color{magenta}{Plan}\color{orange}{ck}}\\
    \bottomrule
    \end{tabular}}
    \caption{Examples of the token routing decisions for the Top-2 routing with load balancing in the math (GSM8K), code (Human Eval), and knowledge (Natural Questions) domains. Tokens highlighted are routed to the following experts: \color{red}{Wikipedia and \textsc{LLaMa-2 7B}}, \color{magenta}{Math and \textsc{LLaMa-2 7B}}, \color{orange}{Code and \textsc{LLaMa-2 7B}}, \color{teal}{Math and Code}, \color{blue}{Wikipedia and Math}, \color{cyan}{Wikipedia and Code}. \color{black}{Tokens that were routed to the in-domain expert are underlined.}}
    \label{table:token_routing}
\end{table*}
